TimEHR: Image-based Time Series Generation for Electronic Health Records

Time series in Electronic Health Records (EHRs) present unique challenges for generative models, such as irregular sampling, missing values, and high dimensionality. In this paper, we propose a novel generative adversarial network (GAN) model, TimEHR, to generate time series data from EHRs. In particular, TimEHR treats time series as images and is based on two conditional GANs. The first GAN generates missingness patterns, and the second GAN generates time series values based on the missingness pattern. Experimental results on three real-world EHR datasets show that TimEHR outperforms state-of-the-art methods in terms of fidelity, utility, and privacy metrics.

==> Tables/SOTA.tex <==
% Table generated by Excel2LaTeX from sheet 'SOTA'
\begin{tabular}{cccccccc}
\toprule
Model & \begin{turn}{45}utility evaluation\end{turn} & \begin{turn}{45}privacy evaluation\end{turn} & \begin{turn}{45}EHRs evaluation\end{turn} & \begin{turn}{45}irregularly-sampled\end{turn} & \begin{turn}{45}missingness\end{turn} & \begin{turn}{45}open source\end{turn} & \begin{turn}{45}Architecture\end{turn} \\
\midrule
TimeGAN & Y     & N     & N     & N     & N     & Y     &  \\
DoppelGANger & Y     & Y     & N     & N     & N     & Y     &  \\
TS-Diffusion & Y     & N     & Y     & Y     & Y     & N     &  \\
GT-GAN & Y     & N     & N     & Y     & N     & Y     &  \\
TimeDiff & Y     & Y     & Y     & Y     & Y     & N     &  \\
EHR-Safe & Y     & Y     & Y     & Y     & Y     & N     &  \\
RTSGAN & Y     & N     & Y     & Y     & Y     & Y     &  \\
\midrule
\textbf{TimEHR} & Y     & Y     & Y     & Y     & Y     & Y     &  \\
\bottomrule
\end{tabular}%


==> Tables/ablation.tex <==
% Table generated by Excel2LaTeX from sheet 'Ablation'
\begin{tabular}{ccccc}
\toprule
Dataset & Model & $AUROC_{MIA}$ & $AA_{train}$ & $AA_{test}$ \\
\midrule
\multirow{5}[2]{*}{P12} & TimeEHR wo CWGAN & 0.003(0.001) & 0.001(0.001) & 0.551(0.01) \\
      & TimeEHR wo Pix2Pix & 0.497(0.009) & 0.935(0.009) & 0.937(0.013) \\
      & TimeEHR wo L2 & 0.496(0.012) & 0.957(0.013) & 0.96(0.01) \\
      & TimeEHR & \textbf{0.494(0.01)} & \textbf{0.735(0.017)} & \textbf{0.747(0.015)} \\
      & BL    & \textit{0.5(0.0)} & \textit{0.512(0.01)} & \textit{0.512(0.01)} \\
\midrule
\multirow{5}[2]{*}{P19} & TimeEHR wo CWGAN & 0.124(0.118) & 0.067(0.102) & 0.564(0.018) \\
      & TimeEHR wo Pix2Pix & 0.5(0.006) & 0.936(0.022) & 0.941(0.018) \\
      & TimeEHR wo L2 & 0.499(0.008) & 0.979(0.006) & 0.979(0.008) \\
      & TimeEHR & \textbf{0.499(0.008)} & \textbf{0.721(0.025)} & \textbf{0.736(0.029)} \\
      & BL    & \textit{0.5(0.0)} & \textit{0.518(0.012)} & \textit{0.518(0.012)} \\
\midrule
\multirow{5}[2]{*}{MIMIC-III} & TimeEHR wo CWGAN & 0.223(0.043) & 0.185(0.049) & 0.781(0.076) \\
      & TimeEHR wo Pix2Pix & 0.493(0.019) & 0.9(0.019) & 0.945(0.03) \\
      & TimeEHR wo L2 & 0.495(0.027) & 0.977(0.006) & 0.988(0.006) \\
      & TimeEHR & \textbf{0.488(0.024)} & \textbf{0.733(0.041)} & \textbf{0.837(0.061)} \\
      & BL    & \textit{0.5(0.0)} & \textit{0.669(0.092)} & \textit{0.669(0.092)} \\
\bottomrule
\end{tabular}%


==> Tables/downstream.tex <==
% Table generated by Excel2LaTeX from sheet 'T3_new'
\begin{tabular}{clccccccc}
\toprule
\toprule
      &       & \multicolumn{3}{c}{P12} &       & \multicolumn{3}{c}{P19} \\
\cmidrule{3-5}\cmidrule{7-9}      &       & \textbf{AUROC} & \textbf{AUPRC} & \textbf{F1-Score} &       & \textbf{AUROC} & \textbf{AUPRC} & \textbf{F1-Score} \\
\midrule
\multirow{6}[2]{*}{\begin{sideways}Baselines\end{sideways}} & Transformer & 84.1(0.9) & 48.5(1.3) & 46.3(3.6) &       & 80.6(2.8) & 43.0(3.8) & 42.7(4.4) \\
      & GRU-D & 81.9(2.1) & 46.1(4.7) & 45.1(2.2) &       & 83.9(1.7) & 46.9(2.1) & 43.9(2.1) \\
      & SeFT  & 74.4(1.3) & 30.2(2.5) & 36.7(1.1) &       & 80.9(2.6) & 41.7(3.4) & 25.2(2.8) \\
      & mTAND & 84.2(0.8) & 48.2(3.4) & 45.9(1.8) &       & 84.4(1.3) & 50.6(2.0) & 45.0(2.9) \\
      & IP-Net & 82.6(1.4) & 47.6(3.1) & 46.0(1.9) &       & 84.6(1.3) & 38.1(3.7) & 41.1(2.3) \\
      & Raindrop & 82.8(1.7) & 44.0(3.0) & 45.0(1.3) &       & 87.0(2.3) & \textbf{51.8(5.5)} & 47.3(3.1) \\
\midrule
\multirow{8}[2]{*}{\begin{sideways}Ours\end{sideways}} & DAM   & 85.7(0.6) & 53.6(1.9) & 49.8(1.0) &       & 87.6(2.5) & 48.6(5.5) & 47.7(3.1) \\
      & TEE+DAM & 84.4(1.5) & 50.9(4.0) & 48.6(1.8) &       & 87.5(2.2) & 49.6(5.5) & 48.4(4.5) \\
      & TEE+DAM w AE & \textbf{86.2(0.8)} & 53.6(4.2) & \textbf{51.8(0.6)} &       & \textbf{88.8(2.2)} & 50.3(4.6) & 49.2(3.9) \\
      & TEE+DAM w PP(ML) & 84.9(1.2) & 49.5(5.3) & 48.6(2.3) &       & 87.6(1.8) & 50.0(4.7) & 49.9(1.6) \\
      & TEE+DAM w PP(Single) & 85.8(0.8) & \textbf{53.7(2.5)} & 50.9(1.5) &       & 88.7(1.7) & 50.4(5.1) & 49.4(3.8) \\
      & [TEE w AE]+DAM & 85.8(1.0) & 52.9(3.0) & 51.6(0.8) &       & 88.1(2.6) & 48.9(5.8) & 48.1(4.2) \\
      & [TEE w PP(ML)]+DAM & 85.1(0.4) & 50.3(4.1) & 48.8(1.1) &       & 87.6(2.1) & 49.5(3.6) & 48.7(1.8) \\
      & [TEE w PP(Single)]+DAM & 85.4(1.5) & 52.4(3.5) & 50.6(1.7) &       & 88.1(1.9) & 50.6(4.3) & \textbf{50.4(2.3)} \\
\bottomrule
\bottomrule
\end{tabular}%


==> Tables/fidelity.tex <==
% Error: No range selected.


==> Tables/fidelity2.tex <==
% Error: No range selected.


==> Tables/meanstd-small.tex <==
% Table generated by Excel2LaTeX from sheet 'meanstd-small'
\begin{tabular}{p{9.87em}p{5.605em}ll}
\toprule
Variable & Train & \multicolumn{1}{p{6.13em}}{TimeEHR} & \multicolumn{1}{p{6.13em}}{RTSGAN} \\
\midrule
HR (4.3) & 86.4 (17.3) & 87.4 (12.9) & \multicolumn{1}{p{6.13em}}{89 (17.6)} \\
Urine (27.2) & 103 (99.9) & 98.2 (75.6) & \multicolumn{1}{p{6.13em}}{116 (86.4)} \\
SysABP (42.6) & 120 (22.2) & 119 (17.5) & \multicolumn{1}{p{6.13em}}{118 (18.5)} \\
DiasABP (42.8) & 59.4 (11.7) & 58.7 (9.23) & \multicolumn{1}{p{6.13em}}{58.9 (9.39)} \\
MAP (43) & 79.7 (14.3) & 78.9 (10.9) & \multicolumn{1}{p{6.13em}}{79 (11.2)} \\
ALP (98.3) & 108 (85.3) & 102 (58.8) & \multicolumn{1}{p{6.13em}}{116 (74.4)} \\
Albumin (98.7) & 2.88 (0.647) & 2.91 (0.555) & \multicolumn{1}{p{6.13em}}{3.31 (0.604)**} \\
TroponinT (98.9) & 0.814 (1.54) & 0.646 (0.926) & \multicolumn{1}{p{6.13em}}{2.04 (2.25)**} \\
TroponinI (99.8) & 7.22 (9.04) & 7.35 (6.6) & \multicolumn{1}{p{6.13em}}{2.16 (1.14)**} \\
Cholesterol (99.8) & 153 (40.9) & 142 (39.9)* & 164 (28.2)* \\
\bottomrule
\end{tabular}%


==> Tables/meanstd.tex <==
% Table generated by Excel2LaTeX from sheet 'meanstd'
\begin{tabular}{p{5.605em}cp{5.605em}p{5.395em}ll}
\toprule
Variable & \multicolumn{1}{p{8.235em}}{Missing rate(\%)} & Train & Test  & \multicolumn{1}{p{6.13em}}{TimeEHR} & \multicolumn{1}{p{6.13em}}{RTSGAN} \\
\midrule
HR    & 4.3   & 86.4 (17.3) & 86.3 (17.5) & 87.6 (12.8) & \multicolumn{1}{p{6.13em}}{89 (17.6)} \\
Urine & 27.2  & 103 (99.9) & 108 (106) & 99.3 (76.1) & \multicolumn{1}{p{6.13em}}{116 (86.4)} \\
SysABP & 42.6  & 120 (22.2) & 120 (22.2) & 119 (17.4) & \multicolumn{1}{p{6.13em}}{118 (18.5)} \\
DiasABP & 42.8  & 59.4 (11.7) & 59.8 (11.9) & 58.7 (9.19) & \multicolumn{1}{p{6.13em}}{58.9 (9.39)} \\
MAP   & 43    & 79.7 (14.3) & 80.1 (14.5) & 78.9 (10.9) & \multicolumn{1}{p{6.13em}}{79 (11.2)} \\
ALP   & 98.3  & 108 (85.3) & 102 (70.5) & 103 (60.2) & \multicolumn{1}{p{6.13em}}{116 (74.4)} \\
Albumin & 98.7  & 2.88 (0.647) & 2.91 (0.656) & 2.94 (0.565) & \multicolumn{1}{p{6.13em}}{3.31 (0.604)**} \\
TroponinT & 98.9  & 0.814 (1.54) & 0.871 (1.58) & 0.658 (0.974) & \multicolumn{1}{p{6.13em}}{2.04 (2.25)**} \\
TroponinI & 99.8  & 7.22 (9.04) & 7.54 (10.8) & 7.18 (6.33) & \multicolumn{1}{p{6.13em}}{2.16 (1.14)**} \\
Cholesterol & 99.8  & 153 (40.9) & 154 (39.6) & 139 (39.9)* & 164 (28.2)* \\
\bottomrule
\end{tabular}%


==> Tables/meanstd2.tex <==
% Table generated by Excel2LaTeX from sheet 'meanstd2'
\begin{tabular}{lcccl}
\toprule
Variable & Train & Test  & TimeEHR & \multicolumn{1}{c}{RTSGAN} \\
\midrule
HR    & 86.4 (17.3) & 86.3 (17.5) & 86.3 (12.8) & 89 (17.6) \\
NIDiasABP & 58.1 (14.6) & 58.6 (14.6) & 55.4 (11.3) & 57.4 (10.5) \\
NIMAP & 77 (14.5) & 77.5 (14.4) & 74.1 (10.9) & 77.3 (11.1) \\
NISysABP & 120 (21.2) & 120 (21.2) & 118 (16.4) & 121 (16.5) \\
RespRate & 19.4 (5.07) & 19.4 (5.09) & 19.4 (4.07) & 19.3 (3.77) \\
Temp  & 37.1 (0.829) & 37.1 (0.826) & 37.2 (0.693) & 37 (0.714) \\
DiasABP & 59.4 (11.7) & 59.8 (11.9) & 57.6 (9.25) & 58.9 (9.39) \\
MAP   & 79.7 (14.3) & 80.1 (14.5) & 78.4 (11) & 79 (11.2) \\
SysABP & 120 (22.2) & 120 (22.2) & 120 (17.6) & 118 (18.5) \\
GCS   & 11.4 (4) & 11.4 (3.97) & 12 (3.5) & 11.7 (3.3) \\
ALT   & 222 (501) & 223 (597) & 134 (284) & 325 (523) \\
AST   & 311 (736) & 259 (612) & 188 (367) & 436 (747) \\
Albumin & 2.88 (0.647) & 2.91 (0.656) & 2.93 (0.555) & 3.31 (0.604) \\
Bilirubin & 2.13 (3.13) & 2.05 (3.05) & 1.37 (1.56) & 2.05 (2.37) \\
Lactate & 2.7 (1.9) & 2.68 (1.81) & 2.35 (1.31) & 3.26 (1.89) \\
Cholesterol & 153 (40.9) & 154 (39.6) & 148 (35.7) & 164 (28.2) \\
TroponinI & 7.22 (9.04) & 7.54 (10.8) & 6.94 (6.35) & 2.16 (1.14) \\
TroponinT & 0.814 (1.54) & 0.871 (1.58) & 0.576 (0.887) & 2.04 (2.25) \\
\bottomrule
\end{tabular}%


==> Tables/preliminary-effects.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet11'
\begin{tabular}{cccccccc}
\toprule
\toprule
      &       &       &       & \multicolumn{4}{c}{\textbf{Dataset}} \\
\cmidrule{5-8}      &       &       &       & \textbf{RT-MC} & \textbf{RT-ML} & \textbf{SO} & \textbf{SYN} \\
\multicolumn{3}{c}{\textbf{TEE}} &       & \textbf{F1-Score} & \textbf{AUROC} & \textbf{F1-Score} & \textbf{AUROC} \\
\cmidrule{1-3}\cmidrule{5-8}\textbf{Loss} & \textbf{w} & \textbf{time_enc} &       &       &       &       &  \\
\cmidrule{1-3}\multirow{8}[8]{*}{AE} & \multirow{2}[2]{*}{3} & concat &       & \textbf{0.63} & 0.71(0.02) & \textbf{0.36(0.01)} & \textbf{0.90(0.00)} \\
      &       & sum   &       & 0.62  & 0.69(0.03) & 0.36(0.01) & 0.89(0.01) \\
\cmidrule{2-8}      & \multirow{2}[2]{*}{2} & concat &       & \textbf{0.63} & 0.71(0.02) & \textbf{0.37(0.01)} & \textbf{0.90(0.01)} \\
      &       & sum   &       & 0.62  & 0.69(0.02) & 0.35(0.02) & 0.89(0.01) \\
\cmidrule{2-8}      & \multirow{2}[2]{*}{1} & concat &       & \textbf{0.63} & 0.70(0.03) & \textbf{0.38(0.02)} & \textbf{0.90(0.01)} \\
      &       & sum   &       & 0.61  & 0.69(0.03) & 0.34(0.01) & 0.86(0.06) \\
\cmidrule{2-8}      & \multirow{2}[2]{*}{0} & concat &       & 0.59  & 0.66(0.03) & 0.32(0.01) & 0.84(0.05) \\
      &       & sum   &       & 0.59  & 0.66(0.03) & 0.33(0.00) & 0.87(0.03) \\
\midrule
\multirow{8}[8]{*}{PP(ML/MC)} & \multirow{2}[2]{*}{3} & concat &       & 0.53  & \textbf{0.74(0.01)} & 0.33(0.01) & 0.58(0.02) \\
      &       & sum   &       & 0.35  & 0.72(0.01) & 0.33(0.01) & 0.59(0.05) \\
\cmidrule{2-8}      & \multirow{2}[2]{*}{2} & concat &       & 0.52  & \textbf{0.74(0.01)} & 0.33(0.01) & 0.60(0.02) \\
      &       & sum   &       & 0.35  & 0.72(0.01) & 0.32(0.00) & 0.61(0.04) \\
\cmidrule{2-8}      & \multirow{2}[2]{*}{1} & concat &       & 0.53  & \textbf{0.74(0.02)} & 0.32(0.00) & 0.60(0.05) \\
      &       & sum   &       & 0.45  & 0.71(0.02) & 0.32(0.00) & 0.60(0.05) \\
\cmidrule{2-8}      & \multirow{2}[2]{*}{0} & concat &       & 0.44  & 0.66(0.03) & 0.32(0.01) & 0.57(0.06) \\
      &       & sum   &       & 0.44  & 0.66(0.03) & 0.32(0.00) & 0.61(0.05) \\
\midrule
\multirow{8}[8]{*}{PP(single)} & \multirow{2}[2]{*}{3} & concat &       & 0.57  & 0.71(0.02) & 0.37(0.01) & 0.65(0.04) \\
      &       & sum   &       & 0.56  & 0.68(0.04) & 0.35(0.00) & 0.65(0.05) \\
\cmidrule{2-8}      & \multirow{2}[2]{*}{2} & concat &       & 0.53  & 0.70(0.03) & 0.38(0.01) & 0.65(0.05) \\
      &       & sum   &       & 0.54  & 0.68(0.03) & 0.35(0.01) & 0.64(0.06) \\
\cmidrule{2-8}      & \multirow{2}[2]{*}{1} & concat &       & 0.57  & 0.70(0.03) & 0.36(0.01) & 0.64(0.04) \\
      &       & sum   &       & 0.54  & 0.68(0.03) & 0.34(0.00) & 0.64(0.04) \\
\cmidrule{2-8}      & \multirow{2}[2]{*}{0} & concat &       & 0.56  & 0.66(0.03) & 0.33(0.00) & 0.62(0.05) \\
      &       & sum   &       & 0.32  & 0.66(0.03) & 0.33(0.00) & 0.62(0.04) \\
\bottomrule
\bottomrule
\end{tabular}%


==> Tables/preliminary2.tex <==
% Table generated by Excel2LaTeX from sheet 'PRE'
\begin{tabular}{ccccccc}
\toprule
\toprule
      &       &       & \multicolumn{4}{c}{\textbf{Dataset}} \\
\cmidrule{4-7}      &       &       & \textbf{RT-MC} & \textbf{RT-ML} & \textbf{SO} & \textbf{SYN} \\
\multicolumn{3}{c}{\textbf{Model}} & \textbf{F1-Score} & \textbf{AUROC} & \textbf{F1-Score} & \textbf{AUROC} \\
\midrule
\multicolumn{3}{c}{Latent} & 0.58  & NR    & 0.28(0.19) & NR \\
\multicolumn{3}{c}{SAHP} & 0.54  & NR    & 0.24  & NR \\
\multicolumn{3}{c}{THP} & 0.54  & NR    & 0.24  & NR \\
\multicolumn{3}{c}{GRU-CP} & NR    & 0.61  & 0.33  & 0.85 \\
\multicolumn{3}{c}{TEE with AE loss} & \textbf{0.63} & 0.70(0.03) & \textbf{0.38(0.02)} & \textbf{0.90(0.01)} \\
\multicolumn{3}{c}{TEE with PP(ML/MC)} & 0.53  & \textbf{0.74(0.02)} & 0.32(0.00) & 0.60(0.05) \\
\multicolumn{3}{c}{TEE with PP(single)} & 0.57  & 0.70(0.03) & 0.36(0.01) & 0.64(0.04) \\
\bottomrule
\bottomrule
\end{tabular}%


==> Tables/privacy.tex <==
% Error: No range selected.


==> Tables/self-sup.tex <==
% Table generated by Excel2LaTeX from sheet 'T2_new'
\begin{tabular}{ccp{6.84em}p{6.5em}p{7.895em}p{7.945em}}
\toprule
\toprule
      &       & \multicolumn{1}{c}{} & \multicolumn{3}{p{22.34em}}{\textbf{Metric}} \\
\cmidrule{4-6}\multicolumn{1}{p{4.13em}}{\textbf{Dataset}} & \multicolumn{1}{p{4.13em}}{\textbf{Loss}} & \textbf{Model} & \textbf{LL/\#events\newline{}(Future Event)} & \textbf{AUROC\newline{}(Future Event)} & \textbf{AUPRC\newline{}(Label)} \\
\midrule
\multicolumn{1}{c}{\multirow{6}[6]{*}{P12}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{PP(ML)}} & TEE   & -2.51(0.03) & 78.79(0.71) & 27.68(2.53) \\
      &       & TEE+DAM & -2.48(0.41) & 74.69(13.80) & 25.13(6.17) \\
\cmidrule{2-6}      & \multicolumn{1}{c}{\multirow{2}[2]{*}{AE}} & TEE   & NA    & 81.62(0.32) & 28.72(2.82) \\
      &       & TEE+DAM & NA    & 84.61(0.70) & 28.59(1.48) \\
\cmidrule{2-6}      & \multicolumn{1}{c}{\multirow{2}[2]{*}{PP(single)}} & TEE   & -1.35(0.02) & 82.34(0.26) & 30.49(2.04) \\
      &       & TEE+DAM & \textbf{-1.33(0.02)} & \textbf{84.84(0.77)} & \textbf{30.93(2.93)} \\
\midrule
\multicolumn{1}{c}{\multirow{6}[6]{*}{P19}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{PP(ML)}} & TEE   & -1.72(0.09) & 76.81(1.06) & 12.21(1.86) \\
      &       & TEE+DAM & -1.42(0.12) & 77.75(1.61) & 24.19(7.57) \\
\cmidrule{2-6}      & \multicolumn{1}{c}{\multirow{2}[2]{*}{AE}} & TEE   & NA    & 90.42(0.33) & 17.79(4.13) \\
      &       & TEE+DAM & NA    & \textbf{92.30(0.08)} & 26.90(3.12) \\
\cmidrule{2-6}      & \multicolumn{1}{c}{\multirow{2}[2]{*}{PP(single)}} & TEE   & -0.71(0.05) & 90.31(0.32) & 19.41(2.65) \\
      &       & TEE+DAM & \textbf{-0.58(0.03)} & 91.11(0.54) & \textbf{28.99(4.07)} \\
\bottomrule
\bottomrule
\end{tabular}%

